Geometrization of purely hyperbolic representations in $\text{PSL}_2\Bbb R$

Let $S$ be a surface of genus $g$ at least $2$. A representation $\rho:\pi_1S\longrightarrow \text{PSL}_2\Bbb R$ is said to be purely hyperbolic if its image consists only of hyperbolic elements other than the identity. We may wonder under which conditions such representations arise as holonomy of a hyperbolic cone-structure on $S$. In this work we will characterize them completely, giving necessary and sufficient conditions.

==> preamble.tex <==

\usepackage[utf8]{inputenc} % set input encoding (not needed with XeLaTeX)
\usepackage{geometry} % to change the page dimensions
\geometry{a4paper} % or letterpaper (US) or a5paper or....
\usepackage{graphicx} % support the \includegraphics command and options
\usepackage{booktabs} % for much better looking tables
\usepackage{array} % for better arrays (eg matrices) in maths
\usepackage{paralist} % very flexible & customisable lists (eg. enumerate/itemize, etc.)
\usepackage{verbatim} % adds environment for commenting out blocks of text & for better verbatim
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{decorations.markings}
\usepackage{subfig}
\usepackage{tabularx}
\usepackage{enumitem}
\usepackage{amsmath,amsthm}
\usepackage{amssymb,amsfonts}
\usepackage{fancyhdr} % This should be set AFTER setting up the page geometry
\usepackage{pgf,tikz}
\usepackage{caption}
\usepackage{tikz-cd}
\usepackage{tikzscale}
\usetikzlibrary{patterns}
\usepackage{rotating}





%\pagestyle{fancy} % options: empty , plain , fancy
%\renewcommand{\headrulewidth}{0pt} % customise the layout...
%\lhead{}\chead{}\rhead{}
%\lfoot{}\cfoot{\thepage}\rfoot{}
%
\geometry{a4paper,top=2cm,bottom=2.5cm,left=2.5cm,right=2.5cm,%
          heightrounded,bindingoffset=0mm}
%          

          

\usepackage{color}   %May be necessary if you want to color links
\usepackage{hyperref}
\hypersetup{
    colorlinks=true, %set true if you want colored links
    linktoc=all,     %set to all if you want both sections and subsections linked
    linkcolor=blue,  %choose some color if you want links to stand out
    citecolor=blue,
    filecolor=blue,
    urlcolor=blue
}


%%%%% BIBLIOGRAPHY
\usepackage[T1]{fontenc}
%\usepackage[american]{babel}
\usepackage{csquotes}
% When using prefixed numerical labels, the labels must be assigned
% as the bibliography is generated. That's why we set
% defernumbers=true here:
\usepackage[style=numeric,defernumbers,backend=bibtex]{biblatex}
\usepackage{hyperref}
\usepackage{nameref}
\addbibresource{biblatex-examples.bib}
% A catch-all filter for all items which are not assigned to a
% dedicated sub-bibliography:
\defbibfilter{other}{
  not type=article
  and
  not type=book
  and
  not type=collection
}

\addbibresource{biblio.bib}





% THEOREMS -------------------------------------------------------
\usepackage{amssymb,amsmath,latexsym,amsthm}
\usepackage{faktor} 		%use as \faktor{A}{B}

\theoremstyle{plain}                    
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem*{thmnn}{Theorem}
\newtheorem{conj}{Conjecture}	
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{ex}[thm]{Example}
\newtheorem*{qs}{Question}
\theoremstyle{remark}
\newtheorem{rmk}[thm]{Remark}

		%not numbered

\numberwithin{equation}{section}



%===COMANDI====

\newcommand{\R}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\hyp}{\mathbb{H}}
\newcommand{\PP}{\mathbb{P}}


\newcommand{\DD}{\mathbb{D}}
\newcommand{\HH}{\mathbb{H}^2}
\newcommand{\HP}{\mathcal{H}^+}
\newcommand{\cp}{\mathbb{C}\mathbb{P}^1}
\newcommand{\rp}{\mathbb{R}\mathbb{P}^1}
\newcommand{\pslc}{\mathrm{PSL}_2\C}
\newcommand{\slc}{\mathrm{SL}_2\C}
\newcommand{\pslr}{\mathrm{PSL}_2\R}
\newcommand{\pglr}{\mathrm{PGL}_2\R}
\newcommand{\wpslr}{\widetilde{\mathrm{PSL}_2\R}}
\newcommand{\psu}{\mathrm{PSU}(1,1)}
\newcommand{\psuu}{\mathrm{PSU}(2)}
\newcommand{\slr}{\mathrm{SL}_2\R}
\newcommand{\qf}{quasi-Fuchsian }
\newcommand{\dev}{\textsf{dev}}
\newcommand{\eu}[1]{\mathcal{E}(#1)}
\newcommand{\eur}[2]{\mathcal{E}(#1,#2)}
\newcommand{\eurr}[4]{\mathcal{E}(#1;#2,#3,#4)}
\newcommand{\x}[1]{\textsf{X}(#1)}
\newcommand{\wrg}{\widetilde{\psi(\gamma)}}
\newcommand{\wrgg}{\widetilde{\psi(g)}}
\newcommand{\wrhh}{\widetilde{\psi(h)}}
\newcommand{\wrgh}{\widetilde{\psi(gh)}}
\newcommand{\gge}{\gamma_\textsf{geod}}
\newcommand{\ggee}{\gamma_\textsf{\emph{geod}}}

\DeclareMathOperator{\sign}{sign}


\newenvironment{sy}%
 {\left\lbrace\begin{array}{@{}l@{}}}%
 {\end{array}\right.}


\newenvironment{mi}[1]%
{\begin{list}{}
         {\setlength{\leftmargin}{#1}}
         \item[]
}
{\end{list}}

\def\qr#1#2{%
      \raise1ex\hbox{$#1$}\Big/ \lower1ex\hbox{$#2$}%
}

\def\qrr#1#2{%
      \raise1ex\hbox{$#1$}\Big/\Big/ \lower1ex\hbox{$#2$}%
}


\def\ql#1#2{%
      \lower1ex\hbox{$#1$}\Big\backslash \raise1ex\hbox{$#2$}%
}

\newenvironment{sistema}%
 {\left\lbrace\begin{array}{@{}l@{}}}%
 {\end{array}\right.}



%===================







